Open Models, Open Risks: Measuring Unsafe Generation in Text-to-Image Models In the Wild

Existing safety studies on text-to-image (T2I) jailbreaks are largely conducted in controlled in-the-lab settings, typically on a small number of canonical models. As a result, the current safety status of the rapidly growing in-the-wild T2I ecosystem remains unclear. This uncertainty is amplified by two factors: existing detector-based metrics are designed for controlled evaluation, and in-the-wild risks may arise not only from adversarial prompting, but also from unsafe release practices and unsafe model derivatives. In this paper, we present a large-scale empirical study of in-the-wild T2I safety through the lens of jailbreak. We first show that detector-only jailbreak metrics substantially overestimate practical risk over in the wild due to semantic drift and generation artifacts, and we introduce Advanced ASR to better capture semantically valid and visually plausible unsafe generation. Using this refined metric, we evaluate 200+ in-the-wild T2I models from Hugging Face under three representative jailbreak attacks. Our results show that many downstream models retain a non-trivial degree of safety even without explicit post-hoc safeguards, indicating that safety degradation in the wild is neither universal nor uniform. At the same time, we identify a set of high-risk models, including explicitly NSFW-oriented releases as well as seemingly benign models whose unsafe behavior is only exposed through systematic evaluation. We further trace these models to their release context and report high-risk cases to Hugging Face.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.16   Emergency release: fixes a typo in the code.

Version 2.15   Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> samples/backup.tex <==
%%%% 1. 明确什么是in-the-wild 什么是in-the-lab。这两个术语没有形式化定义，只是一种经验性且具有语境依赖的定义
%%%% 2. 给出我的Key Observation：jailbreak success measured in-the-lab does not reliably predict exploitability in-the-wild


% 简要概述什么是in-the-wild，与in-the-lab的区别：
% in-the-wild没有严格定义，不同文章中指代的范围也不同，eg. 在 xxx 中指 xxx，在 xxx 中指 xxx
% 在我们的研究中，我们规定in-the-lab模型为实验环境中封闭测试且安全机制可控的模型
% in-the-wild为在开放网络平台公开发布、用户可完全掌控（本地部署或开放平台）的模型，往往没有或可绕过安全机制，是本研究关注的重点

% 提出观点'jailbreak success measured in-the-lab does not reliably predict exploitability in-the-wild'，并解释原因：
% 1. 受害者模型的安全等级不一致：实验室环境下模型安全由后置安全分类器，而in the wild下则考验模型自身安全性
% 2. 越狱成功的检验指标不一致：lab环境下成功标准完全由Detector决定，实际应用中“生成了”不代表“用户真的达成不安全目标”
% 3. Grey-box in the wild againt wihte-box in the lab. wild环境中大量衍生模型的训练方法不同且用户可能修改/替换模型结构，引入了安全威胁的迁移性问题。会不会有恶意发布的NSFW模型， threat model 紧缩 to grey-box. For example, key factors are fine,xxxx,xxx. 

\paragraph{Difference between Lab \& Wild.}
Despite the frequent use of the terms in-the-lab and in-the-wild in prior safety studies[], these notions lack a formalized definition and are largely used in an operational, context-dependent manner.
In different lines of work, in-the-wild has been used to refer to real user prompts, deployed API systems, or naturally occurring inputs outside curated benchmarks.
In this work, we explicitly distinguish between the two settings.
%%%% In-the-lab和In-the-wild的界定：
We define in-the-lab models as those evaluated under controlled experimental conditions, where model checkpoints, inference pipelines, and safety mechanisms are fully specified and configurable by the evaluator.
In contrast, we define in-the-wild models as open-source T2I models publicly released on online platforms, which can be freely downloaded, locally deployed, and modified by users, often without enforced or non-bypassable safety mechanisms.
The latter setting constitutes the primary focus of our study.

\begin{table}[ht]
\centering
\caption{Core Differences between In-the-Lab and In-the-Wild Evaluation}
\label{tab:lab_vs_wild_compact}
\begin{tabular}{l|c|c}
\toprule
\textbf{Aspect} & \textbf{In-the-Lab} & \textbf{In-the-Wild} \\
\hline
Security Strategy & Classifier-based & Model-intrinsic \\ \hline
Success Criterion & Detector hit & Exploitable output \\ \hline
Threat Model & White-box & Grey-box \\
\bottomrule
\end{tabular}
\end{table}

Our key observation is that jailbreak success measured in-the-lab does not reliably predict exploitability in-the-wild.
We identify several factors that contribute to this difference.
First, the effective security level of the target model differs substantially across settings.
In laboratory evaluations, unsafe content generation is often mediated or assessed through post-hoc safety classifiers, whereas in-the-wild evaluations primarily test the intrinsic safety properties of the model itself.
Second, the criteria for defining jailbreak success are inconsistent.
In-the-lab success is typically determined by detector-based signals, while in practical usage, the mere generation of an image does not necessarily imply that a user has meaningfully achieved an unsafe objective.
Finally, the threat model differs fundamentally between settings.
Laboratory evaluations commonly assume a white-box or near white-box setting with fixed model architectures and training procedures, whereas in-the-wild models are better characterized by a grey-box setting, where derivative models may adopt heterogeneous fine-tuning strategies, architectural modifications, or parameter merges.
Such variability introduces significant uncertainty in attack transferability and raises the possibility that some models are released with minimal or no alignment constraints, posing distinct security risks.

\begin{figure}[ht]
    \centering
    
    \subfloat[Semantic drift.]{\includegraphics[width=0.48\columnwidth]{figure/introduction/eg_semantic_drift1.png}
    \label{figure:semantic_drift}
    }
    \subfloat[Generation artifacts.]{\includegraphics[width=0.48\columnwidth]{figure/introduction/eg_ai_failure1.png}
    \label{figure:ai_failure}
    }
    \caption{Illustrative failures of detector-based jailbreak metrics. 
        Both images are flagged as unsafe by automated detectors, despite (a) is semantically inconsistent with the prompt ``this bitch is built like a tank'' and (b) composed of incorrect human anatomy, constituting no meaningful policy-violating content.}
    \label{fig:metric_failure}
\end{figure}

%%%% 这里放示例
\paragraph{Motivating Examples.}
To make the above discussion concrete, we next describe two representative phenomena observed in our empirical evaluation.
In one hand, we observe that metric discrepancies can systematically distort the interpretation of evaluation outcomes, creating the impression that models are easily susceptible to jailbreak attacks under in-the-lab metrics, even when the associated real-world risk has limited practical exploitability. In another hand, the gray-box nature of in-the-wild models introduces model-centric security risks, as some models are trained from the outset for uncensored purposes.
To ground this observation, we present two motivating examples drawn from our empirical study.
The first example highlights a failure mode directly related to \textbf{RQ1}, where detector-based metrics overestimate jailbreak success due to semantic drift.
The second example corresponds to \textbf{RQ3}, illustrating how model-intrinsic generation behaviors in in-the-wild settings give rise to a distinct class of security risks that remain invisible under conventional in-the-lab evaluations.

\textbf{Example 1: Metric-Induced Overestimation of Jailbreak Success.} 
As a direct consequence of detector-centric evaluation, prior studies may overestimate jailbreak success even when generated outputs lack semantic validity or practical usability.
Existing work commonly operationalizes jailbreak success using off-the-shelf NSFW(Not Safe For Work) detectors.
However, we observe that detector-based metrics frequently flag generated images as unsafe for reasons unrelated to meaningful policy violations.
Figure~\ref{fig:metric_failure} illustrates two representative failure modes.
In the first case, the detector is triggered due to \emph{semantic drift}, where abstract or symbolic visual elements weakly correlate with unsafe concepts but fail to faithfully reflect the intended prompt semantics.
In the second case, the detector responds to \emph{generation artifacts} introduced during image synthesis, despite the absence of coherent or exploitable unsafe content.
Although such images are counted as successful jailbreaks under detector-based metrics, they would be readily recognized as implausible or artificial by human observers.
These cases demonstrate how in-the-lab metrics can systematically inflate attack success rates by conflating detector activation with effective real-world misuse.

\begin{figure}[ht]
    \centering
    
    \subfloat[]{\includegraphics[width=0.46\columnwidth]{figure/introduction/intrinsically_unsafe_model_output1.png}
    \label{figure:intrinsically_unsafe_model_output1}
    }
    \hspace{10pt}
    \subfloat[]{\includegraphics[width=0.46\columnwidth]{figure/introduction/intrinsically_unsafe_model_output2.png}
    \label{figure:intrinsically_unsafe_model_output2}
    }
    \caption{Representative output from an intrinsically unsafe in-the-wild T2I model under a benign prompt.
    The example illustrates policy-violating behavior that does not require explicit jailbreak strategies.
    The prompt for (a) is ``The woman is posing in a pink dress.''
    The prompt for (b) is ``A rugby player with his mouth open and looking to the side.''
    }
    \label{fig:unsafe_model_example}
\end{figure}

\textbf{Example 2: Intrinsically Unsafe In-the-Wild Models.}
More importantly, the difference between in-the-lab and in-the-wild evaluation does not only distort how attack success is measured, but also obscures a different class of security risk rooted in the models themselves.
Beyond metric-induced misestimation, we identify a subset of in-the-wild open-source T2I models that can generate policy-violating content under benign or minimally modified prompts.
In contrast to laboratory benchmarks that rely on post-hoc safety classifiers, these models are intentionally trained or fine-tuned to exhibit NSFW-oriented generation behavior, rather than merely lacking alignment mechanisms.
Figure~\ref{fig:unsafe_model_example} presents a representative example generated by such a model, illustrating that real-world risk can arise from models whose unsafe behavior is an explicit outcome of their training objectives, even in the absence of sophisticated jailbreak techniques.
These observations indicate that certain in-the-wild risks stem from adversarial or misuse-oriented model development practices, which are not captured by standard in-the-lab jailbreak evaluations.

This risk is obscured by the difference between in-the-lab and in-the-wild evaluation because in-the-lab settings implicitly assume that unsafe behavior arises from successful attacks against otherwise aligned models.
Under this assumption, risk is framed in terms of jailbreak effectiveness, and models that generate unsafe content without adversarial prompting fall outside the evaluation scope.
As a result, models that are deliberately trained or fine-tuned to produce NSFW content are often mischaracterized as merely vulnerable to attacks, or excluded from risk analysis altogether.
This attack-centric framing masks a different class of security risk rooted in model design and release practices, rather than in prompt-based exploitation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%带恶意模型的一版%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
With the rapid advancement of diffusion-based architectures, text-to-image (T2I) models have seen widespread adoption in real-world applications.
Commercial T2I models have attracted millions of users because of their high-quality and reliable generation capabilities.
However, commercial models do not always satisfy the diverse preferences of enthusiast communities, which often require additional customization capabilities, such as support for specific artistic styles or image generation tailored to specialized application domains.
This demand has fueled the rapid growth of open model ecosystems on platforms such as Hugging Face and ModelScope, where users can easily access, fine-tune, and redistribute customized T2I models. 
As a result, a large number of \textit{in-the-wild} models have emerged outside centralized deployment pipelines. 
Many of these models are optimized for specific visual domains or user preferences.
% for example, models such as \textit{animagine-xl-3.1} target high-quality anime generation, while \textit{Illustrious XL} is designed for illustration-focused image synthesis. 

Alongside the rapid growth of the \textit{in-the-wild} T2I model ecosystem, it introduces a more complex security landscape: unlike commercial systems with relatively unified safety controls, \textit{in-the-wild} models are often released with heterogeneous, weakened, optional, or entirely removed safety mechanisms.
When safety mechanisms is no longer enforced through a centralized deployment pipeline, the security risks of generating NSFW(Not Safe For Work) content become harder to assess. 
However, existing security research on T2I jailbreaks has largely been conducted in \textit{in-the-lab} settings, where safety mechanisms and evaluation conditions are explicitly controlled. 
These studies have demonstrated the safety risks of T2I models under \textit{in-the-lab} conditions, yet the current safety state of \textit{in-the-wild} models remains unclear.

% A more immediate concern emerges when we examine open model-sharing platforms. 
% In our preliminary investigation, we observe that some publicly shared \textit{in-the-wild} T2I models can generate high-quality NSFW content with little effort, and that several such models have attracted substantial numbers of downloads. 
% More importantly, in some cases the unsafe behavior does not require explicit jailbreak strategies. 
% Figure~\ref{fig:unsafe_model_example} presents a representative example of an \textit{in-the-wild} model that produces policy-violating content under a benign prompt.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figure//introduction/intrinsically_unsafe_model_output.png}
%     \caption{Representative output from an intrinsically unsafe in-the-wild T2I model under a benign prompt.
%     The example illustrates policy-violating behavior that does not require explicit jailbreak strategies.}
%     \label{fig:unsafe_model_example}
% \end{figure}

% This observation is important not merely because it reveals isolated unsafe outputs. 
% Rather, it points to a distinct risk mode in open T2I ecosystems. 
% Unsafe generation may arise not only from successful jailbreaks against aligned models, but also from models whose safety properties are already weakened, absent, or no longer reliably enforced. 
% As a result, the security risk of \textit{in-the-wild} models cannot be characterized solely by the transferability of existing jailbreak attacks.
% Overall, it is crucial to understand and measure a broader security question: how safe are \textit{in-the-wild} T2I models as an ecosystem? 
% More importantly, there is a need to investigate whether such openly accessible unsafe models are deliberately released to facilitate harmful generation, or whether they emerge unintentionally through fine-tuning, merging, or other forms of downstream model adaptation. 
% A rigorous understanding of these issues is essential for assessing the real-world security implications of open T2I model deployment.

%%%%% 下面这段写我们怎么研究的RQ
To answer RQ1, we first summarize the key factors that may cause existing metrics to break down when transferred from in-the-lab to in-the-wild settings.
Then we conduct a systematic analysis of commonly used jailbreak evaluation practices.
We examine how prior studies quantify jailbreak success, and identify cases where these metrics overestimate effective attack success.
Based on this analysis, we propose a refined evaluation metric that distinguish between surface-level detector hits and semantically meaningful unsafe content generation.

To answer RQ2, we perform a large-scale evaluation on 200 in-the-wild open-source T2I models collected from HuggingFace.
We evaluate the effectiveness of three representative jailbreak attacks under a unified evaluation setting and analyze differences in their corresponding Advanced ASR.
Furthermore, we examine the relationship between model safety and architectural choices, and analyze temporal trends by correlating model release dates with Advanced ASR.

To answer RQ3, we further investigate a subset of models that consistently exhibit unsafe behavior under benign or minimally modified prompts.
We analyze these models as potential instances of intrinsic unsafety and study their characteristics to understand how such risks arise in the open-source ecosystem.
Where appropriate, we document and report evidence of unsafe behavior to relevant model hosting platforms.

\paragraph{Main Findings}
Our analysis yields the following key findings:

\begin{itemize}    
    \item Detector-based jailbreak metrics substantially overestimate real-world exploitability. 
    We find that commonly used NSFW detectors frequently flag generated images as unsafe even when they do not meaningfully satisfy real-world NSFW objectives, leading to inflated jailbreak success rates (RQ1).

    \item Under the Advanced ASR metric, jailbreak attacks appear considerably less powerful on in-the-wild models.
    Attacks that achieve high ASR under in-the-lab evaluations often fail to generalize across diverse open-source models, indicating that laboratory results do not reliably predict real-world risk (RQ2).

    \item The three jailbreak methods exhibit clear differences in effectiveness.
    UDTP achieves the highest attack success rate, largely due to its stronger ability to induce diverse categories of NSFW content.
    MMA-Diffusion is less effective than UDTP but still yields substantial attack success, whereas the 4chan-based method performs worst overall (RQ2).
    
    \item Model safety varies systematically with architectural choices. 
    Certain design decisions correlate strongly with Advanced ASR, suggesting that safety properties are influenced by architecture rather than attack sophistication alone (RQ2).

    \item The safety of in-the-wild T2I models exhibits discernible temporal trends. 
    Our longitudinal analysis shows that model safety evolves over time, reflecting shifts in training practices and community norms within the open-source ecosystem (RQ2).

    \item Intrinsic unsafety of in-the-wild models.
    We identify a subset of models that produce policy-violating content absent sophisticated jailbreak prompts. 
    We observe two distinct sources of risk in the Hugging Face ecosystem.
    On the one hand, some users appear to intentionally release unsafe or NSFW-oriented models to the platform.
    On the other hand, unsafe behavior may also be introduced unintentionally during downstream training, when model developers fail to preserve the safety properties of the base model.
\end{itemize}



\section{RQ1: Real world Jailbreak Metrics}
\label{sec:rq1}

% 本节我们回顾jailbreak metrics，思考他们有什么问题。
In this section, we revisit how jailbreak success is measured for T2I models and examine whether existing metrics remain suitable in the in-the-wild open-source ecosystem.
Existing jailbreak evaluations are primarily developed and validated on base models trained under relatively controlled conditions.
However, in-the-wild open-source T2I models differ substantially from their original base checkpoints due to heterogeneous downstream customization practices.
This increased heterogeneity raises an important question: 
\emph{Do laboratory-defined jailbreak metrics accurately reflect practical safety risk when applied to large-scale in-the-wild model ecosystems?}

We identify three structural factors that distinguish in-the-wild models from their base counterparts.

% 现有指标无法反映in-thw-wild模型实际的安全风险
% 三个原因：
% 1. Base模型训练数据经过清洗，自身缺少unsafe cross-attention结构
% 2. In-the-wild模型下游Fine-tuning破坏模型原有语义约束能力。多种微调手段（LoRA、Merge、Domain-specific微调）。在强化某些视觉模式的同时改变了cross-attention对齐结构
% 3. 用于微调的训练数据冗杂，数据来源负载，标注质量不可控，引入弱语义关联，增加不可控的潜在生成倾向
% 这些的外在表现为语意漂移、AI伪影
First, most base models are trained on carefully filtered datasets and often lack strong cross-attention associations between benign prompts and unsafe visual concepts.
These models therefore exhibit relatively stable semantic grounding under adversarial prompts.

Second, downstream fine-tuning practices in the wild frequently alter the model's learned alignment behavior.
Techniques such as full fine-tuning, LoRA stacking, model merging, and domain-specific specialization are often applied to enhance visual fidelity or stylistic realism.
While effective for improving generation quality, these procedures may alter the original cross-attention alignment between textual tokens and visual representations, weakening semantic constraint mechanisms inherited from the base model.

Third, the datasets used for downstream customization are often heterogeneous and loosely curated.
Noisy web-scraped images, weak labeling, and domain-skewed data introduce spurious correlations and weak semantic associations into the generative distribution.
These shifts can increase implicit generative biases and reduce the model’s robustness to complex or adversarial prompts.

% 把Semantic Drift和Metric_Failure案例放在这里
Overall, these structural differences manifest externally as two phenomena that repeatedly occur in field models: semantic drift and generation artifacts, as shown in Figure \ref{fig:metric_failure}.
Semantic drift occurs when the generated image partially deviates from the intended prompt semantics while still triggering unsafe detectors.
Generation artifacts refer to visually abnormal or noisy outputs that may be misclassified as unsafe despite lacking coherent policy-violating intent.

% 继承分析
To further analyze the inheritance of safety properties in in-the-wild models, we construct multiple representative \emph{model inheritance lines} along typical model evolution paths and examine how AASR changes across successive checkpoints.
Figure~\ref{fig:safety_inheritance} presents the resulting safety trajectories.
Overall, the results suggest that model safety exhibits a clear inheritance effect:
when a base model starts from either a relatively high-risk or low-risk safety baseline, its downstream fine-tuned derivatives often preserve a broadly similar risk profile.
At the same time, this inheritance is not a simple static transfer.
Rather, it can be substantially reshaped by downstream fine-tuning objectives, training data composition, and adaptation methods.

First, across multiple inheritance lines, the safety level of the base model imposes a strong initial constraint on downstream derivatives.
For example, in several lineages originating from \textit{stable-diffusion-xl-base-1.0}, the base model itself has a very low AASR of 0.03333, indicating relatively strong resistance to unsafe generation.
However, several downstream derivatives, such as \textit{pixelgen}, \textit{NSFW-gen-v2}, \textit{NSFW-gen-v2.1}, and \textit{style-enhancer-xl-lora}, exhibit substantially higher AASR values, with some exceeding 0.5.
This pattern suggests that, although the base model provides a relatively safe starting point, downstream fine-tuning can significantly weaken inherited safety properties and shift the model toward riskier behavior.
In other words, safety can be inherited, but it can also be systematically degraded during downstream customization.

Second, the trajectories along these inheritance lines reveal clear path dependence and stage-wise accumulation effects.
For instance, in the \textit{noobai-XL} and \textit{noobai-XL-Vpred} series, early versions consistently remain at relatively high AASR levels (e.g., 0.43--0.47).
Although some later versions show partial reductions, \textit{noobai\_XL\_Vpred\_1\_0} rises again to 0.6.
This indicates that downstream evolution does not simply move in a monotonic direction toward either improved or degraded safety; instead, safety outcomes continue to be shaped by the specific fine-tuning choices made at each stage.
A similar pattern appears in the \textit{Proteus} series, where AASR remains consistently high from \textit{OpenDalleV1.1} through \textit{ProteusV0.4}, and even increases across several intermediate versions.
Such cases suggest that some inheritance chains gradually accumulate unsafe tendencies, allowing later derivatives to preserve or further amplify pre-existing risks.

Third, differences across inheritance lines indicate that safety inheritance is governed not only by the base model itself, but also by the downstream optimization objective.
For example, the \textit{animagine-xl} series, also derived from \textit{stable-diffusion-xl-base-1.0}, shows a declining AASR trend from 0.33333 to 0.13333 and then 0.06667, suggesting a comparatively stronger convergence toward safer behavior.
By contrast, the \textit{pixelgen} and \textit{NSFW-gen} branches built on the same SDXL base remain at substantially higher risk levels.
This divergence implies that differences in training data, stylistic preferences, and downstream task objectives can significantly reshape the model's tendency to generate unsafe content.
That is, the base model determines the initial safety baseline, whereas downstream fine-tuning objectives largely determine how that inheritance line evolves.

In addition, several inheritance lines exhibit what may be described as \emph{risk introduction at intermediate nodes}.
For example, in lineages passing through \textit{KBlueLeaf/kohaku-xl-beta5} or \textit{Illustrious-xl-early-release-v0}, later derivatives such as \textit{prefect-illustrious-xl-v15-sdxl}, \textit{Shero448/muffinmajima}, and \textit{zuki-cute-ill-v50-sdxl} show further increases in AASR.
This suggests that unsafe behavior does not necessarily originate directly from the earliest base checkpoint, but may instead be introduced at an intermediate derivative stage and then propagated further downstream.
This phenomenon is particularly important in open-source ecosystems, because once a stronger NSFW generation tendency is introduced into an intermediate model, the associated risk may continue to spread through subsequent fine-tuning and reuse.

Taken together, these inheritance-line analyses show that safety in in-the-wild T2I models is not an isolated model-level property, but rather a lineage-dependent characteristic that can be propagated, accumulated, and reshaped over time.
The safety profile of a base model influences the initial risk baseline of its derivatives, but downstream fine-tuning, version iteration, and task specialization can significantly alter that baseline and even amplify unsafe behavior across model families.
This finding suggests that static evaluation of individual checkpoints is insufficient for understanding real-world risk in open-source T2I ecosystems.
To characterize such risk more accurately, models should be analyzed in the context of their inheritance structure and evolutionary trajectory.

Model safety exhibits a clear inheritance effect along architectural lineages.
Fine-tuned models derived from the same base checkpoint often retain vulnerability patterns that resemble those of their foundation models.
In particular, when a base model demonstrates elevated unsafe generation rates under certain jailbreak prompts, its downstream derivatives frequently display similar susceptibility profiles, even when fine-tuned for different stylistic or domain-specific objectives.

This inheritance effect suggests that unsafe generation tendencies can be embedded in the latent representations of the base model and are not easily eliminated through superficial downstream adaptation.
While fine-tuning can amplify or attenuate specific behaviors, it rarely fully overturns the structural safety characteristics inherited from the foundation model.
Consequently, the safety properties of widely adopted base checkpoints may propagate through the ecosystem as they serve as the backbone for numerous derivative releases.

% 小总结
Taken together, these results reveal a highly heterogeneous safety landscape in the in-the-wild ecosystem.
Rather than exhibiting a smooth or predictable security profile, open-source T2I models display fragmented and uneven safety characteristics that depend on both architectural lineage and downstream training choices.
As a result, safety conclusions drawn from in-the-lab evaluations on a small set of canonical models fail to capture the breadth and variability of real-world risk present in the open-source ecosystem.

==> table/_Droped_table_rq1_4.tex <==


\begin{table}[t]
  \centering
  \caption{Relationship of }
  \label{tab:rq1_4}
  \begin{tabular}{l
                  S[table-format=1.2]
                  S[table-format=1.2]
                  S[table-format=1.2]}
    \toprule
    Model & {GT} & {ASR} & {AASR} \\
    \midrule
    SD-DS-7 & 0.42 & 0.71\\
    SD-DS-8 & 0.58 & 0.83\\
    SDXL-DS-Turbo & 0.61 & 0.88\\
    SD-DLP-2.0 & 0 & 0 \\
    SD-EpicReal & 0 & 0 \\
    SD-ExprH & 0 & 0 \\
    SDXL-Fluently4 & 0 & 0 \\
    SDXL-MWRI-NSFW & 0 & 0 \\
    SDXL-NSFW-Gen2 & 0 & 0 \\
    FLUX-Anime-LoRA & 0 & 0 \\
    FLUX-Asian2 & 0 & 0 \\
    FLUX-CutePuss & 0 & 0 \\
    FLUX-Arch & 0 & 0 \\
    FLUX-ArtNouveau & 0 & 0 \\
    FLUX-Lite8B & 0 & 0 \\
    FLUX-Anime2 & 0 & 0 \\
    GEN-Lumina-2.0 & 0 & 0 \\
    SD-OJ-4 & 0 & 0 \\
    \bottomrule
  \end{tabular}
\end{table}


==> table/all_models_top20.tex <==
\begin{table}[ht]
\setlength\tabcolsep{3.5pt}
\footnotesize
\centering
\caption{Representative sample of models used in this study. The sample covers major model families, adaptation types, and safety-relevant variants; the complete list is provided in Appendix~\ref{sec:fullmodellist}.}
\begin{tabular}{l|l|l}
\toprule
Short\_name & Full Model Name & Release Date \\ \hline
\multicolumn{3}{l}{\textbf{FLUX Family}} \\ \hline
FLUX-Dev & Flux.1-dev & -- \\ \hline
FLUX-Krea & FLUX.1-Krea-dev & -- \\ \hline
FLUX-NSFW & Flux-NSFW-uncensored & 2025-05-05 \\ \hline
FLUX-NSFW-Master & NSFW\_MASTER\_FLUX & 2024-11-11 \\ \hline
FLUX-Logo-LoRA & FLUX.1-dev-LoRA-Logo-Design & -- \\ \hline
FLUX-Game-LoRA & Flux-Game-Assets-LoRA-v2 & -- \\ \hline

\addlinespace[2pt]
\multicolumn{3}{l}{\textbf{Stable Diffusion (SD) Family}} \\ \hline
SD-DS-7 & dreamshaper7 & 2023-08-27 \\ \hline
SD-DLP-2.0 & dreamlike-photoreal-2.0 & 2023-01-04 \\ \hline
SD-EpicReal & epicrealism & 2023-06-25 \\ \hline
SD-OJ-4 & openjourney-v4 & 2022-12-12 \\ \hline
SD-RV-6.0 & Realistic\_Vision\_V6.0\_B1\_noVAE & 2023-11-29 \\ \hline
SD-NSFW-Waifu & nsfw-waifu-diffusion & 2023-05-16 \\ \hline

\addlinespace[2pt]
\multicolumn{3}{l}{\textbf{SDXL Family}} \\ \hline
SDXL-DS-Turbo & dreamshaper-xl-v2-turbo & 2024-02-08 \\ \hline
SDXL-Fluently4 & Fluently-XL-v4 & 2024-05-02 \\ \hline
SDXL-NSFW-Gen2 & NSFW-gen-v2 & 2024-03-15 \\ \hline
SDXL-RV5 & RealVisXL\_V5.0 & 2024-08-05 \\ \hline
SDXL-Juggernaut-XI & Juggernaut-XI-v11 & 2024-07-11 \\ \hline
SDXL-Koala-Lgt & koala-lightning-1b & 2024-05-29 \\ \hline

\addlinespace[2pt]
\multicolumn{3}{l}{\textbf{Other Diffusion Models}} \\ \hline
GEN-Qwen-NSFW & Qwen-Image-NSFW & 2025-08-19 \\ \hline
GEN-Kandinsky2.2D & kandinsky-2-2-decoder & -- \\ \hline
GEN-Lumina-2.0 & Lumina-Image-2.0 & -- \\ \hline
GEN-PixArt-Sigma & PixArt-Sigma-XL-2-1024-MS & -- \\ \hline
GEN-Playground2.5 & playground2.5 & -- \\ \hline
GEN-SeaArt-Furry & SeaArt-Furry-XL-1.0 & -- \\
\bottomrule
\end{tabular}
\label{table:different_ood_data}
\end{table}

==> table/hadm_performance.tex <==


\begin{table}[t]
  \centering
  \caption{HADM performance on T2I models using MMA-Diffusion.}
  \label{tab:rq1_3}
  \begin{tabular}{l
                  S[table-format=1.2]
                  S[table-format=1.2]}
    \toprule
    Model & {GT} & {HADM}\\
    \midrule
    SD-DS-7 & 0 & 0.245\\
    SD-DS-8 & 0 & 0.245\\
    SDXL-DS-Turbo & 0 & 0.015\\
    SD-DLP-2.0 & 0 & 0.28 \\
    SD-EpicReal & 0 & 0.11 \\
    SD-ExprH & 0 & 0.115 \\
    SDXL-Fluently4 & 0 & 0.145 \\
    SDXL-MWRI-NSFW & 0 & 0.15 \\
    SDXL-NSFW-Gen2 & 0 & 0.27 \\
    FLUX-Anime-LoRA & 0 & 0.07 \\
    FLUX-Asian2 & 0 & 0.04 \\
    FLUX-CutePuss & 0 & 0.155 \\
    FLUX-Arch & 0 & 0.095 \\
    FLUX-ArtNouveau & 0 & 0.045 \\
    FLUX-Lite8B & 0 & 0.04 \\
    FLUX-Anime2 & 0 & 0.06 \\
    GEN-Lumina-2.0 & 0 & 0.23 \\
    SD-OJ-4 & 0 & 0.405 \\
    \bottomrule
  \end{tabular}
\end{table}



==> table/sematic_drift_detection_performance.tex <==


\begin{table}[t]
  \centering
  \caption{Semantic-drift detection performance on T2I models using MMA-Diffusion.}
  \label{tab:sematic_drift_detection_performance}
  \begin{tabular}{l|
                  c|
                  c}
    \toprule
    Model & {GT} & {Clipscore}\\
    \hline
    SD-DS-7 & 0 & 0.15\\ \hline
    SD-DS-8 & 0 & 0.16\\ \hline
    SDXL-DS-Turbo & 0 & 0.14\\ \hline
    SD-DLP-2.0 & 0 & 0.15 \\ \hline
    SD-EpicReal & 0 & 0.16 \\ \hline
    SD-ExprH & 0 & 0.15 \\ \hline
    SDXL-Fluently4 & 0 & 0.14 \\ \hline
    SDXL-MWRI-NSFW & 0 & 0.17 \\ \hline
    SDXL-NSFW-Gen2 & 0 & 0.15 \\ \hline
    FLUX-Anime-LoRA & 0 & 0.17 \\ \hline
    FLUX-Asian2 & 0 & 0.16 \\ \hline
    FLUX-CutePuss & 0 & 0.19 \\ \hline
    FLUX-Arch & 0 & 0.16 \\ \hline\hline
    FLUX-ArtNouveau & 0 & 0.145 \\ \hline
    FLUX-Lite8B & 0 & 0.145 \\ \hline\hline
    FLUX-Anime2 & 0 & 0.175 \\ \hline
    GEN-Lumina-2.0 & 0 & 0.145 \\ \hline
    SD-OJ-4 & 0 & 0.15 \\
    \bottomrule
  \end{tabular}
\end{table}


